Rethinking Sketching as Sampling: A Graph Signal Processing Approach

Sampling of signals belonging to a low-dimensional subspace has well-documented merits for dimensionality reduction, limited memory storage, and online processing of streaming network data. When the subspace is known, these signals can be modeled as bandlimited graph signals. Most existing sampling methods are designed to minimize the error incurred when reconstructing the original signal from its samples. Oftentimes these parsimonious signals serve as inputs to computationally-intensive linear operators. Hence, interest shifts from reconstructing the signal itself towards approximating the output of the prescribed linear operator efficiently. In this context, we propose a novel sampling scheme that leverages graph signal processing, exploiting the low-dimensional (bandlimited) structure of the input as well as the transformation whose output we wish to approximate. We formulate problems to jointly optimize sample selection and a sketch of the target linear transformation, so when the latter is applied to the sampled input signal the result is close to the desired output. Similar sketching as sampling ideas are also shown effective in the context of linear inverse problems. Because these designs are carried out off line, the resulting sampling plus reduced-complexity processing pipeline is particularly useful for data that are acquired or processed in a sequential fashion, where the linear operator has to be applied fast and repeatedly to successive inputs or response signals. Numerical tests showing the effectiveness of the proposed algorithms include classification of handwritten digits from as few as 20 out of 784 pixels in the input images and selection of sensors from a network deployed to carry out a distributed parameter estimation task.

==> backward-sketching.tex <==
%!TEX root = ./sketching.tex

%\vspace{\lessss}

This section presents the optimal sampling $\bbC^{*}\in \ccalC_{np}$ and sketching $\bbH_{s}^{*}\in \reals^{m \times p}$ solutions for the inverse problem in Fig. \ref{fig_backward} {and Section~\ref{sssec_prob_inverse}}. Paralleling the structure of the previous section, we first analyze the particular case where the observations are noise free, then shift to the general noisy case, and finally look at a suboptimal scheme where the sketch is formed by taking \textit{rows} of the linear transformation $\bbH^{T}$. Since proof arguments are similar to those used for the direct sketching problem, we skip the details that can be found in~\cite{FGAMGMAR_globalsip16}.

\subsection{Noisy case} \label{subsec_noisy_backward}

As in Section \ref{subsec_noisy_forward} we consider that the noise $\bbw \in \reals^{n}$ is independent of $\bbx$, has zero mean and that its covariance matrix satisfies $\bbR_{w}\succ \bbzero$. Upon defining $\bbG=\bbH^{T}\bbA_{\mathrm{LS}}$, the next proposition characterizes the optimal $\bbC^*$ and $\bbH_{s}^*$ matrices.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   P   O   S   I   T   I   O   N   %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proposition} \label{prop_noisy_backward_x}
If $\bbH$ is full rank, the solution to problem \eqref{eqn_backward_sketching} is given by $\bbC^{*}$ and $\bbH_s^{*}=\bbH_s^{*}(\bbC^{*})$, where

\begin{equation}\label{eqn_H2_noisy_backward_x}
    \bbH_s^{*}(\bbC) = \bbA_\mathrm{LS} \bbR_{x} \bbC^{T} \left( \bbC ( \bbR_{x}+\bbR_{w}) \bbC^{T} \right)^{-1}.
\end{equation}
%
The optimum selection matrix $\bbC^{*}$ is obtained from solving

\begin{equation} \label{eqn_prob1_backward_x}
   \min_{\bbC \in \ccalC_{np}} \ \tr \big[ \bbR_{x} - \bbG \bbR_{x} \bbC^{T} \left( \bbC (\bbR_{x}+\bbR_{w}) \bbC^{T} \right)^{-1} \bbC \bbR_{x} \bbG^{T} \big].
\end{equation}
%
\end{proposition}
%

As was the case for the direct problem, the joint design of the optimal selection matrix $\bbC^{*}$ and the optimal sketch $\bbH_{s}^{*}$ can be carried out as a two-step process. First $\bbC^*$ is found as the solution to \eqref{eqn_prob1_backward_x}, which only requires as input $\bbR_{x}$, $\bbG$ and $\bbR_{w}$. Then, the optimal sketch is found using \eqref{eqn_H2_noisy_backward_x} $\bbH_{s}^{*}=\bbH_{s}^{*}(\bbC^{*})$.

Moreover, note that the optimal sketch $\bbH_s^{*}$ is tantamount to the LS operator $\bbA_\mathrm{LS}=(\bbH\bbH^{T})^{-1}\bbH$ acting on a preprocessed version of $\bbx$, via the matrix $\bbR_{x} \bbC^{T} ( \bbC (\bbR_{x}+\bbR_{w}) \bbC^{T} )^{-1}$. What this preprocessing entails is, essentially, choosing the samples of $\bbx$ with the optimal tradeoff between the signal in the multiplicative term $\bbR_{x} \bbC^{T}$ and the noise in the inverse term $( \bbC (\bbR_{x}+\bbR_{w}) \bbC^{T} )^{-1}$. Also observe that, while computation of the inverse-mapping sketch $\bbH_{s}^{*}$ involves the (costly) computation of $(\bbH \bbH^{T})^{-1}$, this is carried out entirely off line.

Finally, the optimization problem \eqref{eqn_prob1_backward_x} over $\bbC$ is equivalent to a problem reminiscent of an SDP save the binary constraints, as shown next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   P   O   S   I   T   I   O   N   %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proposition} \label{prop_noisy_backward_x_sdp}
In the setting of Proposition \ref{prop_noisy_backward_x}, the optimum selection matrix $\bbC^{*}$ is such that the diagonal elements $\bbc^{*}$ of $(\bbC^{*})^{T}\bbC^{*}=\diag(\bbc^{*})$, are given by the solution to the problem

\begin{align}
  \min_{\substack{\bbc \in \{0,1\}^{n},\\\bbY, \barbC_{\alpha}}}\
	& \tr \left[ \bbY \right] \label{eqn_prob2_backward_x} \\
    \st
	 &\: \barbC_{\alpha} = \alpha^{-1}\diag(\bbc) \ , \ \bbc^{T} \bbone_{n} = p \nonumber \\
	& \begin{bmatrix} \bbY - \bbR_{x} + \bbG \bbR_{x} \barbC_{\alpha}\bbR_{x} \bbG^{T} & \bbG \bbR_{x} \barbC_{\alpha} \\ \barbC_{\alpha} \bbR_{x} \bbG^{T} & \barbR_{\alpha}^{-1}+\barbC_{\alpha} \end{bmatrix} \succeq \bbzero,
		\nonumber 
\end{align}
%
where $\barbR_{\alpha}=(\bbR_{x}+\bbR_{w}-\alpha \bbI_{n})$, $\barbC_{\alpha}$ and $\bbY\in \reals^{n\times n}$ are auxiliary variables and $\alpha>0$ is any scalar satisfying $\barbR_{\alpha}\succ \bbzero$.
\end{proposition}
%

%\vspace{\lessss}

\subsection{Sampling the linear transformation} \label{subsec_hsampling_backward}

Here we look at setups where the sketch $\bbH_{s}$ is constrained to be a submatrix of $\bbH$. In the context of linear inverse problems, this amounts to saying that $\bbH_{s}=\bbH \bbC^{T}$ is formed using $p$ columns of $\bbH$. With $\barbH=\bbH^{T} \bbH$ denoting the $n \times n$ Gram matrix of $\bbH$, the solution to \eqref{eqn_backward_sketching} for sketches of the form $\bbH_{s}=\bbH \bbC^{T}$ is given by the following proposition.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   P   R   O   P   O   S   I   T   I   O   N   %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proposition} \label{prop_hsampling_backward_x}
	Let $\bbH_{s}=\bbH \bbC^{T}$ be constructed from a subset of $p$ columns of $\bbH$. Then, the optimal sampling matrix $\bbC^{*}$ can be recovered from vector $\bbc^{*}$ that contains the diagonal elements of $(\bbC^{*})^{T} \bbC^* = \diag(\bbc^{\ast})$, where $\bbc^{*}$ is the solution to the following problem
	
	\begin{align}
		\min_{\substack{\bbc \in \{0,1\}^{n},\\\bbY, \barbC}}\
		& \tr [\bbY] \label{eqn_prob2_hsampling_backward_x} \\
		\st\
		& \barbC=\diag(\bbc) \ , \ \bbc^{T} \bbone_{n} = p \nonumber \\
		& \begin{bmatrix} \bbY - \bbR_{x} + 2 \barbH \barbC \bbR_{x} & \barbH \barbC \\ \barbC \barbH & (\bbR_{x}+\bbR_{w})^{-1} \end{bmatrix} \succeq \bbzero.
		\nonumber
	\end{align}
	%
\end{proposition}

